Synthesis of Opacity-Enforcing Winning Strategies Against Colluded Opponent

This paper studies a language-based opacity enforcement in a two-player, zero-sum game on a graph. In this game, player 1 (P1) wins if it can achieve a secret temporal goal described by the language of a finite automaton, no matter what strategy the opponent player 2 (P2) selects. In addition, P1 aims to win while making its goal opaque to a passive observer with imperfect information. However, P2 colludes with the observer to reveal P1's secret whenever P2 cannot prevent P1 from achieving its goal, and therefore, opacity must be enforced against P2. We show that a winning and opacity-enforcing strategy for P1 can be computed by reducing the problem to solving a reachability game augmented with observer's belief states. Furthermore, if such a strategy does not exist, winning for P1 must entail the price of revealing his secret to the observer. We demonstrate our game-theoretic solution of opacity-enforcement control through a small illustrative example and in a robot motion planning problem.

==> Images/Winning_states.tex <==
\begin{table}[htp!]
\centering
\caption{The winning states for robot A.}
\begin{tabular}{|c|c|c|c|c|c|}
\hline 
 \diagbox{r}{c}&
  0 &
  1 &
  2 &
  3 &
  4 \\ \hline
0 &
  B wins &
  B wins &
  B wins &
  B wins &
  B wins \\ \hline
1 &
  \begin{tabular}[c]{@{}c@{}}A wins \\  opacity\end{tabular} &
  B wins &
  B wins &
  B wins &
  B wins \\ \hline
2 &
  A wins &
  \begin{tabular}[c]{@{}c@{}}A wins\\   opacity\end{tabular} &
  B wins &
  B wins &
  B wins \\ \hline
3 &
  \begin{tabular}[c]{@{}c@{}}A wins\\   opacity\end{tabular} &
  A wins &
  \begin{tabular}[c]{@{}c@{}}A wins\\   opacity\end{tabular} &
  B wins &
  B wins \\ \hline
4 &
  A wins &
  \begin{tabular}[c]{@{}c@{}}A wins \\  opacity\end{tabular} &
  A wins &
  \begin{tabular}[c]{@{}c@{}}A wins\\   opacity\end{tabular} &
  B wins \\ \hline

\end{tabular}

\end{table}

==> co-safeLTL.tex <==
 The objective is defined using a \ac{scltl} formula.
 %
\begin{definition}[\ac{scltl} \cite{kupferman2001model}]
 Given a set of atomic propositions $\calAP $, a syntactically co-safe Linear Temporal Logic (LTL) formula over $\calAP$ is defined using the following grammer
\[ \varphi := \top \mid \bot \mid p \mid \neg p \mid  \varphi \land \varphi \mid \varphi \vee \varphi \mid \Next \varphi \mid \varphi_1 \Until \varphi_2 \mid \Eventually \varphi \] where $\top,\bot$ are universally true and false, respectively, $p \in \calAP$ is an atomic proposition, $\neg$, $\land$ and $\vee$ are the Boolean operators \textit{negation}, \textit{disjunction}, and \textit{conjunction}, respectively, and $\Next, \Until$ and $\Eventually $ denote the temporal operators \textit{next}, \textit{until} and \textit{eventually}, respectively.\end{definition}

%  \begin{definition}[\ac{ltl} \cite{kupferman2001model}]
%  Let $\calAP $ be a set of atomic propositions, the Linear Temporal Logic (LTL) has the following syntax 
% \[ \varphi := \top \mid \bot \mid p \mid \varphi \mid \neg\varphi \mid \varphi_1 \land \varphi_2 \mid \Next \varphi \mid \varphi_1 \Until \varphi_2 \mid \Eventually \varphi \] where $\top,\bot$ are universally true and false, respectively, $p \in \calAP$ is an atomic proposition, $\Next, \Until$ and $\Eventually $ denote the temporal modal operators for \textit{next}, \textit{until} and \textit{eventually}.\end{definition}

%A co-safe \ac{ltl} formula contains only the temporal operator $\Next$, $\Until$, and $\Eventually$ and must be written in positive normal form, \textit{i.e.} negation of temporal operator is not allowed \cite{kupferman2001model}. 

A co-safe \ac{ltl} formula can be equivalently represented by a \ac{dfa} defined as $\mathcal{A} = ( Q, \Sigma, \delta, \init, F )$, where $Q$ is the set of states, $\calAP$ is the set of atomic propositions, $\Sigma= 2^{\calAP}$ is the set of input symbols, $\delta: Q\times \Sigma \rightarrow Q$ is a deterministic transition function, $\init$ is the initial state and $F \subseteq Q$ is the set of accepting states. A word  $w=w_0w_1\ldots w_n \in \Sigma^\ast$  is accepted by $\cal A$ if and only if $\delta(\init, w)\in F$.

An infinite word $w\in \Sigma^\omega$ satisfying an \ac{scltl} formula $\varphi$  if and only if it has a \emph{good} finite prefix $\hat{w}=w_0w_1\ldots w_n$ that is accepted by the \ac{dfa} corresponding to $\varphi$.
%
Note that in this case, for any infinite word $w' \in \Sigma^*$, $\hat{w} w'$ satisfies $\varphi$.
%
 Given a co-safe \ac{ltl} formula, the \ac{dfa} accepting finite good prefixes for $\varphi$ can be obtained using standad tools such as Spot~\cite{duret2016spot,duret2022spot}. 
 %
 We will assume that all \ac{dfa}s referred to in this paper are complete, i.e. for every state $q \in Q$ and for every input symbol $a \in \Sigma$ the transition function $\delta(q, a)$ is defined. An incomplete \ac{dfa} can be made complete by introducing a sink state and directing all undefined transitions into the sink state. 
 \hr{
  By Hopcroft's book~\cite{hopcroft2001introduction}, a DFA has always a complete transition function, so I think we may omit this part. 
  %
  Or in the definition of the DFA, we just say that $\delta$, which is a complete function, is a transition function.
 }

==> grid_world.tex <==
We consider another robot motion planning example (Fig.~\ref{fig:initial_state}). Consider a 5 $\times$ 5 grid world. There are two robots on the field. One is an aerial robot P1 and the other is a ground robot P2. They both have 4 actions $\{N, S, W, E\}$ representing moving north, south, west, and east, respectively. If they move onto the same cell, robot P2 can intercept P1 and the game is over. However, there are 9 cells in the middle representing the water area, where the ground robot is unable to enter but the aerial robot can. The initial position of robot P2 is fixed at $(0,0)$. We consider different initial positions of robot P1 to evaluate if P1 has winning and opacity-enforcing winning strategies from different initial game states.

The goal of robot P1 is to collect 3 samples $G_0, G_1, G_2$ on the field. The sample $G_0$ is required to be collected first. The sample $G_1$, and $G_2$ are the same, robot P1 can collect either of them. The goal can be written as $\Eventually G_0 \land (G_0 \to \Eventually (G_1 \lor G_2))$.  


\begin{figure}%
\centering
\includegraphics[scale=0.25]{Images/Winning Region Encoding.png} 
\caption{The opacity-enforcing winning states.}
    % \subfloat[\centering Example of a state of the game.]{{\includegraphics[width=4.5cm]{Images/The_Covert operation_of_UAV.png} }}%
    % \subfloat[\centering The opacity-enforcing winning states.]{{\includegraphics[width=4.5cm]{Images/Winning Region Encoding.png} }}%
    % \caption{The covert operation of aerial robot}%
    \label{fig:initial_state}%
\end{figure}


\aknote{Removing Fig. 6a.}
Besides the two robots, there is a monitor P3 who is to determine if  the goal of P1 is achieved or not. P3 partially observes the field through sensors. There are two kinds of sensors in the grid world.
\begin{itemize}
    \item[1.] In each row of the grid world, there is a sensor, which returns 1 if the robot is in its row, and 0 otherwise.
    \item[2.] Robot P2 holds a sensor with a sensor range of the cross. Once robot P1 enters the range of the sensor, monitor P3 will get the exact position of P1.
\end{itemize}

P2's goal is to prevent P1 from completing the task and in case P2 cannot do so, P2 wants to reveal to P3 that P1 achieves the goal by using its sensor and environment sensors to provide informative observations to P3.
%The goal of robot P2 is also to keep the samples safe. P2 can make it in two ways. 1. Intercept robot P1 before it collects the samples. 2. Reveal the mission of robot P1. Once monitor P3 knows the mission, P3 can report it. And then P1's mission fails. Therefore, robot P1 needs to complete the mission in secret.
